LatentKeypointGAN: Controlling Images via Latent Keypoints

Generative adversarial networks (GANs) have attained photo-realistic quality in image generation. However, how to best control the image content remains an open challenge. We introduce LatentKeypointGAN, a two-stage GAN which is trained end-to-end on the classical GAN objective with internal conditioning on a set of space keypoints. These keypoints have associated appearance embeddings that respectively control the position and style of the generated objects and their parts. A major difficulty that we address with suitable network architectures and training schemes is disentangling the image into spatial and appearance factors without domain knowledge and supervision signals. We demonstrate that LatentKeypointGAN provides an interpretable latent space that can be used to re-arrange the generated images by re-positioning and exchanging keypoint embeddings, such as generating portraits by combining the eyes, nose, and mouth from different images. In addition, the explicit generation of keypoints and matching images enables a new, GAN-based method for unsupervised keypoint detection.

==> tex/supp_editing.tex <==
\section{More Editing} \label{sec:more_comparison}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/integral_0.jpg}
\end{center}
   \caption{\textbf{Editing on FFHQ.} \textbf{The 1st column}: original image; \textbf{the 2nd column}: part appearance source image used to swap part appearance; \textbf{the 3rd column}: the combined image with shape from the original images and the appearance from the part appearance source image; \textbf{the 4th column}: only changing eyes; \textbf{the 5th column}: only changing mouth; \textbf{the 6th column}: only changing nose; \textbf{the 7th column}: scaling the face 0.85x down; \textbf{the 8th column}: scaling the face 1.15x up; \textbf{the 9th column}: move eyes closer; \textbf{the 10th column}: move eyes farther; \textbf{the 11th column}: move the face to the left and add another one on the right; 
   }
\label{fig:more_editing}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/integral_15.jpg}
\end{center}
   \caption{\textbf{Editing.} 
   }
  \label{fig:more_editing2}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/integral_30.jpg}
\end{center}
   \caption{\textbf{Editing.} 
   }
   \label{fig:more_editing3}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/integral_45.jpg}
\end{center}
   \caption{\textbf{Editing.} 
   }
   \label{fig:more_editing4}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/integral_60.jpg}
\end{center}
   \caption{\textbf{Editing.} 
   }
   \label{fig:more_editing5}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/integral_75.jpg}
\end{center}
   \caption{\textbf{Editing.} 
   }
   \label{fig:more_editing6}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/integral_90.jpg}
\end{center}
   \caption{\textbf{Editing.} 
   }
   \label{fig:more_editing7}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/removing_0.jpg}
\end{center}
   \caption{\textbf{Removing keypoints one by one.} We remove the keypoints one by one for faces in Figure~\ref{fig:more_editing}. The first column shows the original image without removing any keypoints.
   }
\label{fig:removing}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/removing_15.jpg}
\end{center}
   \caption{\textbf{Removing keypoints one by one.} We remove the keypoints one by one for faces in Figure~\ref{fig:more_editing2}.
   }
\end{figure*}

% \begin{figure*}
% \begin{center}
% \includegraphics[width=0.98\linewidth]{images/more_editing/removing_30.jpg}
% \end{center}
%   \caption{\textbf{Removing keypoints one by one.} We remove the keypoints one by one for faces in Figure~\ref{fig:more_editing3}.
%   }
% \end{figure*}

% \begin{figure*}
% \begin{center}
% \includegraphics[width=0.98\linewidth]{images/more_editing/removing_45.jpg}
% \end{center}
%   \caption{\textbf{Removing keypoints one by one.} We remove the keypoints one by one for faces in Figure~\ref{fig:more_editing4}.
%   }
% \end{figure*}

%----------------------------------------eye interpolation--------------------------------------

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/eyes_0.jpg}
\end{center}
   \caption{\textbf{Keypoint appearance embedding interpolation.} We show the interpolation of eyes for faces in Figure~\ref{fig:more_editing}. \textbf{The 1st column}: original image; \textbf{the 2rd-8th column}: the interpolation from the original images to the part source images; \textbf{the 9th column}: part appearance source image used to swap part appearance;; \textbf{the 10th column}: the difference between the original images and the swapped images.
   }
\label{fig:eye_interpolation}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/eyes_15.jpg}
\end{center}
   \caption{\textbf{Keypoint appearance embedding interpolation.} We show the interpolation of eyes for faces in Figure~\ref{fig:more_editing}. \textbf{The 1st column}: original image; \textbf{the 2rd-8th column}: the interpolation from the original images to the part source images; \textbf{the 9th column}: part appearance source image used to swap part appearance;; \textbf{the 10th column}: the difference between the original images and the swapped images.
   }
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/eyes_30.jpg}
\end{center}
   \caption{\textbf{Keypoint appearance embedding interpolation.} We show the interpolation of eyes for faces in Figure~\ref{fig:more_editing2}.
   }
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/eyes_45.jpg}
\end{center}
   \caption{\textbf{Keypoint appearance embedding interpolation.} We show the interpolation of eyes for faces in Figure~\ref{fig:more_editing3}.
   }
\end{figure*}

%----------------------------------------mouth interpolation--------------------------------------

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/mouth_0.jpg}
\end{center}
   \caption{\textbf{Keypoint appearance embedding interpolation.} We show the interpolation of mouths for faces in Figure~\ref{fig:more_editing}. \textbf{The 1st column}: original image; \textbf{the 2rd-8th column}: the interpolation from the original images to the part source images; \textbf{the 9th column}: part appearance source image used to swap part appearance; \textbf{the 10th column}: the difference between the original images and the swapped images.
   }
\label{fig:mouth_interpolation}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/mouth_15.jpg}
\end{center}
   \caption{\textbf{Keypoint appearance embedding interpolation.} We show the interpolation of mouths for faces in Figure~\ref{fig:more_editing1}.
   }
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/mouth_30.jpg}
\end{center}
   \caption{\textbf{Keypoint appearance embedding interpolation.} We show the interpolation of mouths for faces in Figure~\ref{fig:more_editing2}.
   }
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/mouth_45.jpg}
\end{center}
   \caption{\textbf{Keypoint appearance embedding interpolation.} We show the interpolation of mouths for faces in Figure~\ref{fig:more_editing3}.
   }
\end{figure*}

%----------------------------------------nose interpolation--------------------------------------

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/nose_0.jpg}
\end{center}
   \caption{\textbf{Keypoint appearance embedding interpolation.} We show the interpolation of noses for faces in Figure~\ref{fig:more_editing}. \textbf{The 1st column}: original image; \textbf{the 2rd-8th column}: the interpolation from the original images to the part source images; \textbf{the 9th column}: part appearance source image used to swap part appearance;; \textbf{the 10th column}: the difference between the original images and the swapped images.
   }
\label{fig:nose_interpolation}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/nose_15.jpg}
\end{center}
   \caption{\textbf{Keypoint appearance embedding interpolation.} We show the interpolation of noses for faces in Figure~\ref{fig:more_editing2}.
   }
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/nose_30.jpg}
\end{center}
   \caption{\textbf{Keypoint appearance embedding interpolation.} We show the interpolation of noses for faces in Figure~\ref{fig:more_editing3}.
   }
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/nose_45.jpg}
\end{center}
   \caption{\textbf{Keypoint appearance embedding interpolation.} We show the interpolation of noses for faces in Figure~\ref{fig:more_editing4}.
   }
\end{figure*}

%----------------------------------------BBCPose-------------------------------------------
\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/bbcpose_0.jpg}
\end{center}
   \caption{\textbf{Editing on BBCPose}. 
   }
\end{figure*}

%----------------------------------------Bedroom-------------------------------------------
\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/bedroom_0.jpg}
\end{center}
   \caption{\textbf{Editing on LSUN Bedroom} \textbf{The 1st column}: original image; \textbf{the 2rd column}: part source images; \textbf{the 3th column}: swapping all parts; \textbf{the 4th column}: changing bed; \textbf{the 5th column}: removing bed.
   }
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/bedroom_30.jpg}
\end{center}
   \caption{\textbf{Editing on LSUN Bedroom}. 
   }
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/bedroom_failure_0.jpg}
\end{center}
   \caption{\textbf{Failure cases on LSUN Bedroom}. 
   }
\end{figure*}

%----------------------------------------comparison-------------------------------------------
\section{More Comparison with SEAN} \label{sec:more_comparison}
\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/comparison_0.jpg}
\end{center}
   \caption{\textbf{Qualitative comparison with SEAN \cite{zhu2020sean}} The first five columns show our results and the last five columns show the results of SEAN \cite{zhu2020sean}. \textbf{Note that for SEAN, the first and the second columns are reconstructed image instead of edited images.} For two combined columns: \textbf{The 1st column}: original image; \textbf{the 2nd column}: part appearance source image used to swap appearance; \textbf{the 3rd column}: the combined image with shape from the original images and the appearance from the part appearance source image; \textbf{the 4th column}: only changing mouth \& jaw; \textbf{the 5th column}: only changing eyes.
   }
\label{fig:more_comparison}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/comparison_15.jpg}
\end{center}
   \caption{\textbf{Qualitative comparison with SEAN \cite{zhu2020sean}}
   }
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/comparison_30.jpg}
\end{center}
   \caption{\textbf{Qualitative comparison with SEAN \cite{zhu2020sean}}
   }
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/comparison_45.jpg}
\end{center}
   \caption{\textbf{Qualitative comparison with SEAN \cite{zhu2020sean}}
   }
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/comparison_60.jpg}
\end{center}
   \caption{\textbf{Qualitative comparison with SEAN \cite{zhu2020sean}}
   }
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/comparison_75.jpg}
\end{center}
   \caption{\textbf{Qualitative comparison with SEAN \cite{zhu2020sean}}
   }
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.98\linewidth]{images/more_editing/comparison_90.jpg}
\end{center}
   \caption{\textbf{Qualitative comparison with SEAN \cite{zhu2020sean}}
   }
\end{figure*}


